Towards Ideal Temporal Graph Neural Networks: Evaluations and Conclusions after 10,000 GPU Hours

Temporal Graph Neural Networks (TGNNs) have emerged as powerful tools for modeling dynamic interactions across various domains. The design space of TGNNs is notably complex, given the unique challenges in runtime efficiency and scalability raised by the evolving nature of temporal graphs. We contend that many of the existing works on TGNN modeling inadequately explore the design space, leading to suboptimal designs. Viewing TGNN models through a performance-focused lens often obstructs a deeper understanding of the advantages and disadvantages of each technique. Specifically, benchmarking efforts inherently evaluate models in their original designs and implementations, resulting in unclear accuracy comparisons and misleading runtime. To address these shortcomings, we propose a practical comparative evaluation framework that performs a design space search across well-known TGNN modules based on a unified, optimized code implementation. Using our framework, we make the first efforts towards addressing three critical questions in TGNN design, spending over 10,000 GPU hours: (1) investigating the efficiency of TGNN module designs, (2) analyzing how the effectiveness of these modules correlates with dataset patterns, and (3) exploring the interplay between multiple modules. Key outcomes of this directed investigative approach include demonstrating that the most recent neighbor sampling and attention aggregator outperform uniform neighbor sampling and MLP-Mixer aggregator; Assessing static node memory as an effective node memory alternative, and showing that the choice between static or dynamic node memory should be based on the repetition patterns in the dataset. Our in-depth analysis of the interplay between TGNN modules and dataset patterns should provide a deeper insight into TGNN performance along with potential research directions for designing more general and effective TGNNs.

==> 8_response.tex <==
\section{Response to reviewer comments}
We thank the reviewers for their critical assessment of our work. We first highlight the major improvements and new experiment details.
Then, we address the reviewers' concerns point by point.

\subsection{Highlights in Revised Paper}
The highlights in the revised paper are:
\begin{enumerate}[label=\arabic*:, leftmargin=0.44cm]
\item \textbf{Introduction of new datasets}: We have included the results from two large-scale datasets, \textit{GDELT}~\cite{tgl} and \textit{SuperUser}~\cite{orca}. Our datasets highlight considerable scales and diversity:
\begin{enumerate}
    \item Scale of the datasets: Among the nine datasets in our experiments, four have over a million edges, and \textit{GDELT}~\cite{tgl} has hundreds of millions of edges.
    \item Diversity of the datasets: Our datasets include social networks from multiple online platforms(\textit{Wikipedia}~\cite{jodie}, \textit{REDDIT}~\cite{jodie}, \textit{UCI}~\cite{opsahl2009clustering}, \textit{CollegeMsg}~\cite{panzarasa2009patterns}, and \textit{LASTFM}~\cite{jodie}), user action network (\textit{MOOC}~\cite{jodie}), transportation network (\textit{Flights}~\cite{edgebank}), and global events knowledge graph(\textit{GDELT}~\cite{tgl}).
\end{enumerate}

In Section~\ref{sec:res}, we have included results and conclusions on these datasets. We have examined certain claims regarding the cost-effectiveness of modules on these large datasets in Section ~\ref{subsec:conn}.

\item \textbf{Taxonomy of DGNN network}: We have added a taxonomy of Dynamic Graph Neural Networks (DGNNs) in Section~\ref{sec:intro}, including the definitions of Continuous Time Dynamic Graphs (CTDGs) and Discrete Time Dynamic Graphs (DTDGs) and methods designed for them. Existing TGNN frameworks have also been introduced and compared to ours, which helps readers position our work in the scope and distinguish our contribution from other works.

\item \textbf{Discussion on scalable training techniques}: We have revised our work to include recent advancements in scalable TGN training and to facilitate the deployment of these acceleration techniques within our research framework. Specifically, we have added a discussion in Section ~\ref{subsec:modular} about recent adaptive sampling methods, such as ASTGN~\cite{astgn} and TASER~\cite{taser}, and the possibility of incorporating these methods as a comparison. Additionally, we have discussed distributed training frameworks, like DistTGL~\cite{disttgl} and GNNFlow~\cite{gnnflow}, which can be used to accelerate our modular TGNN framework. We provided guidelines in Section ~\ref{subsec:hs} for multi-GPU configurations to support future integration and evaluation of distributed optimizations.

\item \shepherding{ \textbf{Discussions on the datasets}: We have added explanations on the choice of datasets when we display the results and confirmed the universality of our conclusions. Specifically, we have explained that we showed the results on all datasets when possible. When space is limited, we have explained our principals in the selection of datasets to display: For universal results of module comparison, we selected commonly used datasets (like \textit{Wikipedia} and \textit{REDDIT}) with which readers may be more familiar; for results that require a discussion involving dataset patterns, we selected a diverse combination of datasets to provide a comprehensive discussion on the module performance; for analysis about scalability, we select datasets of all scales. }
    
\end{enumerate}

\subsection{Response to Meta-Reviewer}
\begin{enumerate}[label=\arabic*:, leftmargin=0.44cm]
    \item \textbf{The authors should extend the study to some larger temporal datasets, such as those suggested by one of the reviewers, and more diverse ones.}
    
    We have extended our datasets to include larger and more diverse temporal graphs. The scale and diversity of the datasets have been expanded to enhance our experiments:
    \begin{enumerate}
        \item Scale of the datasets: We have introduced \textit{GDELT}~\cite{tgl} and \textit{SuperUser}~\cite{orca}. Among the nine datasets in our experiments, four have over a million edges, and \textit{GDELT}~\cite{tgl} has hundreds of millions of edges.
        \item Diversity of the datasets: Besides social networks from diverse online platforms(\textit{Wikipedia}~\cite{jodie}, \textit{REDDIT}~\cite{jodie}, \textit{UCI}~\cite{opsahl2009clustering}, \textit{CollegeMsg}~\cite{panzarasa2009patterns}, and \textit{LASTFM}~\cite{jodie}), we also have datasets from other domains, including user action dataset (\textit{MOOC}~\cite{jodie}), transportation network (\textit{Flights}~\cite{edgebank}), and global events knowledge graph(\textit{GDELT}~\cite{tgl}).

    \end{enumerate}
    
    \item \textbf{The authors should improve the positioning of their study, possibly with the help of a taxonomy of DGNN networks.}
    To strengthen the positioning of our work among frameworks of DGNNs, we have added the following information in Section ~\ref{sec:intro}: We have added a taxonomy of discrete-time and continuous-time temporal graphs and introduced the methods developed for each type; we have also summarized the focus and highlights of existing DGNN training frameworks. We position our work as a DGNN framework on CTDGs that highlights a unified framework for module evaluation. 
    % This additional information about temporal graph types and existing frameworks enhances the clarity of the introduction and helps readers more effectively position our work within the field.
    
    \item \textbf{The revision should strive to better account for recent works on scalable TGN training (with optimized modules or even new model architecture).}
    
    We have added the following information to account for recent works on scalable TGNN training and to facilitate easier deployment of these acceleration techniques on top of our research:
    \begin{enumerate}
        \item Recent works on adaptive sampling~\cite{astgn, taser} have strived to scale TGN training by adaptively selecting the informative neighbors. They can be included as extra methods in our evaluation of node sampling. We did not include them for comparison because of the complicated formulations and the significant computation and communication overhead induced. We have added a discussion about these works in Section ~\ref{subsec:modular} and left a more thorough comparison for future work.
        \item Some works ~\cite{disttgl, gnnflow} have proposed distributed training frameworks for acceleration. The reason why we have not assessed our framework in a distributed setting is three-fold: Distributed training techniques involve designing unique data formats and non-trivial optimizations; they are usually designed for specific types of TGNNs (TGL~\cite{tgl} for memory-based TGNNs, and TGOpt~\cite{tgopt} for accelerating TGAT~\cite{tgat}); our main focus in this work is evaluating the performance and interplay of modules. We added a guideline in Section ~\ref{subsec:hs} for multi-GPU settings, facilitating easier integration and evaluations of optimizations for distributed TGNN training/inference in the future.

    \end{enumerate}
    \item \textbf{\shepherding{Please consider carefully the questions raised about the choices of datasets, by Reviewer 2. Please make these choices clear by adding text in the paper.}}
    
    \shepherding{We have explained our choices of datasets when displaying the results and added comments on the universality of conclusions in Section~\ref{sec:res}.  Specifically, we have included results for all datasets whenever feasible. When space constraints limited the number of datasets displayed, we have outlined the principles guiding our selection: For general module comparison, we prioritized commonly used datasets (e.g., \textit{Wikipedia} and \textit{REDDIT}) to ensure familiarity for readers. For discussions involving dataset-specific patterns, we selected a diverse set of datasets to enable a comprehensive analysis of module performance. For scalability analyses, we chose datasets spanning various scales.}

    \item \textbf{\shepherding{Please use the suggestions of Reviewer 1 (reformulate to reduce the number of lines with one or two words only) in order to make space for the clarifications requested above.
    If any of your justifications do not fit in the format even after these edits, consider publishing a slightly longer version somewhere else, e.g., arXiv, etc., and referring to it in the paper.}}
    
    \shepherding{We have rephrased certain sentences to eliminate single-word or two-word lines, enhancing the overall reading flow and fluency.}
    

    \item \textbf{The authors should do their best effort to answer all the other detailed questions raised by the reviews.}

    We have addressed the detailed concerns of the reviewers to the best of our efforts, as displayed in the following sections.
    
\end{enumerate}

\subsection{Response to Reviewer \#1}

\begin{enumerate}[label=\arabic*:, leftmargin=0.44cm]
    \item \textbf{\uline{D1/O1}: Limited background about temporal graph types and TGNN frameworks: The paper introduces a formulation for temporal Graph Neural Networks (GNNs) and lists the state-of-the-art methods. However, it lacks sufficient information about the types of temporal graphs and the methods designed for various applications, such as discrete-time dynamic graphs and continuous-time dynamic graphs, as explained in ~\cite{gravina2024deep}. The background section would be stronger if the authors provided a taxonomy of TGNN methods and utilized datasets of varying sizes to study these methods. Numerous dynamic GNN training frameworks have been developed to support the training of TGNN models for both discrete-time and continuous-time dynamic graphs, such as PyGT, TGL, and DyGLib, as highlighted in ~\cite{dyglib}. The paper’s contribution would be more compelling if the authors provided a detailed discussion on the differences between the proposed unified pipeline and these existing research efforts.}
    
    To enhance our background on temporal graph types and TGNN frameworks and help better position our work, we have added an introduction to different temporal graph modeling and methods in Section~\ref{sec:intro}. We have added one short paragraph to provide a taxonomy of discrete- and continuous-time temporal graphs (DTDGs and CTDGs) and further introduced methods designed for each. We have explained that our framework is located in the more general domain of CTDGs. 
    
    To help readers better identify the contribution from other TGNN training frameworks, we have summarized the focus of existing dynamic GNN training frameworks and highlight our different focus in Section ~\ref{sec:intro}.

    \item \textbf{\uline{D2/O2}: Small temporal graph datasets and limited temporal graph ML tasks. }
    
    \textbf{\uline{D2.A}: Small temporal graph datasets.
    The datasets used in the study are relatively small. Due to scalability issues, the authors decided to limit the number of edges to a maximum of 1 million by selecting only the most recent 1 million edges (Table 4). However, the authors did not explain why they chose the most recent 1 million edges or how this choice affects the quality of the training dataset. Additionally, the datasets used are primarily small bipartite graphs with at most two node/edge types. It would be valuable to evaluate the pipeline with a larger dataset containing hundreds of millions of edges, such as the GDELT and MAG datasets mentioned in ~\cite{tgl}. Scaling to larger graphs may challenge the paper's claims about the efficiency of neighbor sampling compared to node memory modules.}

    To address the limited scale and diversity of datasets, we have further introduced two large datasets with billions of edges on top of million-edge datasets \textit{LASTFM} and \textit{Flights}: GDELT~\cite{tgl} and SuperUser~\cite{orca}. The nine datasets we experimented on contain five non-bipartite graphs and four bipartite graphs, with social networks(\textit{Wikipedia}~\cite{jodie}, \textit{REDDIT}~\cite{jodie}, \textit{UCI}~\cite{opsahl2009clustering}, \textit{CollegeMsg}~\cite{panzarasa2009patterns}, and \textit{LASTFM}~\cite{jodie}), user action network (\textit{MOOC}~\cite{jodie}), transportation network (\textit{Flights}~\cite{edgebank}), and global events knowledge graph(\textit{GDELT}~\cite{tgl}). The enlarged scale and improved diversity of the datasets further consolidate our claim. We have included the information about the new datasets in Section ~\ref{subsec:task} and Section ~\ref{subsec:datasets}. We have expanded our discussions about the effectiveness of modules on the two new large-scale datasets in Section~\ref{sec:res}. 
    
    When preprocessing these datasets for training and testing, we choose the last 1 million edges (following the work TASER~\cite{taser}) for three reasons: 1. We choose the last 1 million instead of randomly sampling edges because the chronological consistency needs to be maintained for temporal graph datasets so that the density of the graph is minimally affected along the time axis. 2. The number of edges is a hyperparameter that we chose following previous work~\cite{taser}. 3. We ran models on the original and truncated dataset. While we consume significantly more resources on the original dataset, we found no difference in the analysis and preference of the modules. As a result, we chose to exhibit most of our results on the processed dataset.
    
    Regarding the reviewer's concern about the claim on the efficiency comparison of neighbor sampling to node memory modules, we have experimented with the large-scale original dataset, and the results still support our claim. we noticed that while the training time increased for the node memory module because of the large training data, it took a significantly longer time for models depending on pure neighbor sampling to aggregate the messages from a larger neighborhood. 
    
    These discussions and results have been added to Section~\ref{subsec:datasets} and Section ~\ref{subsec:conn}, respectively.
    
    \textbf{\uline{D2.B}: The paper focused solely on the link prediction task. Hence, all claims about the effectiveness of different module combinations were based on this single task type. The paper's contribution would be stronger if the authors included additional tasks, such as node classification and graph classification, as demonstrated in ~\cite{feng2024comprehensive}. This would better support the claims about the universality of module effectiveness (RQ2).}
    
    We acknowledge that introducing additional tasks would strengthen the claims of this work. However, the existing modules and datasets are generally not designed for proper evaluation of node/graph classification for the following reasons: 1. The datasets are not well-established for node/graph classification tasks. For node classification, the label quality (banned/unbanned users) is poor and biased on existing datasets (\textit{Wikipedia} and \textit{REDDIT}). Datasets for temporal graph classification were only recently introduced with TP-GNN~\cite{tpgnn}, published in July, 2024, and the quality of graph classification datasets remains largely untested. 2. In node classification, the lack of supervision has led to a two-stage training pipeline in existing work~\cite{tgl}, where self-supervised link prediction is used to train node embeddings in the first stage, and a classifier is trained in the second stage. This significantly enlarges our design space and leads to more complicated optimization. 
    
    We have introduced the node classification task on all datasets following previous work~\cite{tgl} and discussed the following results.

    \begin{figure}[tb]
    \centering
    \setlength{\abovecaptionskip}{5pt} 
    \setlength{\belowcaptionskip}{-3pt} 
    \input{tikz_figs/all_comb_node}
    \caption{Performance of node classification task with different combinations of TGNN modules on dataset \textit{Wikipedia} and \textit{REDDIT}. We plot the accuracy of node classification with respect to the number of neighbors, with different combinations of modules.}
    \label{fig:reb}
    \end{figure}
    

    The significant standard deviation in Figure~\ref{fig:reb} supports our claims regarding dataset limitations and the challenging optimization setting. We have included this discussion in Section ~\ref{subsec:task} and plan to evaluate other tasks in future work.

    \item \textbf{\uline{D3/O3}: Evaluation results require clarifications and a lack of scalability settings.}
    
    \textbf{\uline{D3.A}: The paper claims about deeper layers and wider sampling inefficiency are widely studied in other papers such as ASTGN ~\cite{astgn}. It would be interesting to show how the different combinations of modules could or could not help to figure out “the valuable part of events that happened over a period of time” to benefit the training and reduce the sampling/aggregations cost.
    }

    As the reviewers mentioned, there are some existing works on dealing with the inefficiency of deeper and wider neighbor sampling through adaptive sampling~\cite{astgn, taser}. These methods did not fully address the problem, for they bring significant computation and communication overheads at runtime. Our work discusses this problem by evaluating the necessity of sampling in deeper and wider neighborhoods in a benchmarking framework, as shown in Section~\ref{subsec:conn}. We have added the discussion about other efficient sampling methods in Section ~\ref{subsec:modular}.
    
    As our focus in this work is to evaluate the TGNN modules, we did not make specific efforts to figure out how combinations of modules help distinguish the valuable part of events over a period. However, we have analyzed how the choice of memory module affects the effective capture of temporal repetition in the datasets. The extensions to test how other sampling, aggregation, and node memory or their combinations may capture valuable events are left for future work. We have added this point to Section ~\ref{sec:future}.
    
    \textbf{\uline{D3.B}: In Figure 2, it would be interesting to explain why UNI-sampling performs better in certain cases, such as in the Reddit dataset with 5, 10, 20, and 50 nodes using mixer+emb, compared to MR-sampling. Correlating these results with the graph structure could provide valuable insights. Additionally, it would be helpful to discuss why the MRR improvement margin is generally higher in Wikidata than in Reddit.}

    In Figure ~\ref{fig:sampling1}, there is an occasional advantage of \textbf{uni} sampler over \textbf{MR} sampler when using \textbf{emb} static node memory. This may be caused by the shared nature of static node embedding and uniform sampling of capturing long-term temporal neighborhoods, resulting in good training dynamics on dataset \textit{REDDIT} with long-term repetitions. We have added explanations about this phenomenon in Section~\ref{subsec:ns}.

    On the MRR improvement margin of \textbf{MR} sampling over \textbf{uni} sampling, the different recency patterns of important events in the temporal neighborhood may account for the larger margin on \textit{Wikipedia} over \textit{REDDIT}. As \textit{Wikipedia} is a dataset with short-term repetitions, \textbf{MR} may be able to capture more relevant events on it, resulting in even better performance. We have added discussions in Section ~\ref{subsec:ns}.

    \textbf{\uline{D3.C}: It would be interesting to explain why the combination atten+RNN+MR is the best in Wikipedia and the third best in REDDIT, and the same for mixer+emb+uni.
    Fixing the number of neighbours on the X-Axis does not reflect the graph connecitiviy (dense vs sparse) impact on the training, it would be better to use the sampler number of hops instead in the X-Axis.
    The two layers GNN did not help. What are possible combinations to improve this behaviour?
    Why MRR with Reddit is increasing but looks steady to decreasing in general with other datasets?
    }

    1. atten+RNN+MR works better on \textit{Wikipedia} than \textit{REDDIT}, which may result from the fact that different dataset repetition patterns lead to a preference for node memory. As we explained in Section ~\ref{subsec:mem}, \textit{Wikipedia} is a dataset with short-term repetition patterns, where \textbf{RNN} node memory works better than \textbf{emb} node memory. On the other hand, \textit{REDDIT} is a dataset with long-term repetition patterns. As a result, \textbf{emb} node memory works better on \textit{REDDIT}, and atten+emb+MR has a better performance than atten+RNN+MR.

    2. All the neighbor sampling methods we evaluate employ layer-wise sampling, which does not involve graph sparsity. Consequently, our experiments do not address the impact of graph connectivity (dense vs. sparse) on training. Instead, we focus primarily on evaluating how the neighborhood size affects model performance. Evaluating the effect of graph connectivity with varying hop numbers will require introducing other sampling methods, which we left for future work.
    
    3. The reason that two-layer TGNNs did not work better may be accounted for by the fact that TGNNs with more layers have larger generalization gaps, as discussed in \cite{cong2024generalization} and in Section~\ref{subsec:ns} of our paper. To reduce the generalization gap, we could employ a node memory module or increase data volume ~\cite{cong2024generalization}.
    
    4. The MRR is increasing on \textit{REDDIT} with the increase of neighbors and hops, but steady or decreasing using certain combinations on some datasets. This effect may be caused by different reasons. On small datasets like \textit{UCI}, the MRR decrease may be caused by overfitting (as shown in Figure 4). On larger datasets like \textit{Flights}, we can observe a steady increase in MRR, probably due to the alleviation of the overfitting issue. On \textit{Wikipedia}, the decrease of some combinations may be caused by the suboptimality. Note that although some combinations have a steady or decreasing performance, the best combination of modules still has a performance gain with the increase of neighbors and hops. 
    
    We have added the discussions in Section ~\ref{sec:res}. 

    \textbf{\uline{D3.D}: The paper claimed that “datasets with long-term repetition patterns have a strong preference towards emb-node memory, while those with short-term repetition patterns tend to favor RNN”. What is the time complexity to calculate such pattern existence specially in large scale datasets using algorithm 1? Do you think it is scalable? How to improve it?
    }

    The complexity of this algorithm is $\mathcal{O}(D^2 |\mathcal{V}|)$, where $D$ is the maximum degree. The complexity can be controlled by clipping the maximum degree, which does not affect our recurrence analysis. This algorithm requires only a one-time computation to reveal the dataset pattern. Thus, we leave potential accelerations for future work and have added the discussion in Section ~\ref{subsubsec:dsrep}.

    \textbf{\uline{D3.E}: The evaluation would be stronger if the authors tested the proposed pipeline under distributed training and inference settings (multi-CPU or multi-GPU). This approach would greatly benefit the assessment of the different module combinations' impact on pipeline scalability ~\cite{feng2024comprehensive}.
    }

    While testing the scalability of the modules would make the evaluation more compelling, it also introduces many data dependency issues~\cite{tgl} that may lead to the inability to capture some correlations among events. Training TGNNs under distributed settings usually requires more optimizations and intricate designs to leverage the resources without embarrassingly parallelizing the algorithms~\cite{tgl, gnnflow}. As the distributed training techniques are usually non-trivial and we have a different focus on evaluating the performance and interplay of modules, we did not evaluate our framework under distributed settings. We added a guideline for deploying our framework in multi-GPU settings in Section ~\ref{subsec:hs}, facilitating easier integration and evaluations of optimizations for distributed TGNN training/inference.

    \item \textbf{\uline{D4}: Minor comments:
    The line colors in the figures are difficult to distinguish. Grouping the lines into color groups and using different line styles would improve clarity.
    Figure 12: The dashed lines are missing.
    The authors optimized existing methods to incorporate them into their pipeline. What are the guidelines for optimizing and incorporating other methods?
    Figure 3: Make RNN+uni dotted lines and RNN+MR solid lines with the same color.}

    We thank the reviewer for carefully reviewing and have made changes accordingly. It is easy to incorporate other methods in our benchmarking framework for it is highly modular. We also added a short guideline in our code repository.

    \item \shepherding{ \textbf{ \uline{AD1}: Additional Comments:
    To improve readability and overall aesthetics, please avoid instances where text ends with a single line or just one or two words. These occurrences can disrupt the flow of the text and detract from the paper’s visual appeal. Also, could you consider using space-efficient techniques for figures to maximize clarity and make sure that visual elements are well integrated with the text? }}

    \shepherding{We thank the reviewer for the detailed comment on improving the readability and have made changes accordingly. Specifically, we adjusted the spacing in Figure ~\ref{fig:sampling2} and Figure ~\ref{fig:aggr} to make them more compact, and we changed the coloring in Figure ~\ref{fig:emb-strategy} for enhanced clarity.}    

\end{enumerate}

\subsection{Response to Reviewer \#2}

\begin{enumerate}[label=\arabic*:, leftmargin=0.44cm]
\item \textbf{\uline{D1/W2}: The evaluation could be improved by using larger temporal graph datasets, such as AskUbuntu, SuperUser, and Wiki-Talk (the datasets used in the paper\cite{orca}).}

We have expanded our temporal graph datasets to include two large graph datasets, GDELT~\cite{tgl} and SuperUser~\cite{orca}. We have included the information about the new datasets in Section ~\ref{subsec:task} and Section ~\ref{subsec:datasets}. We have expanded our discussions about the effectiveness of modules on the two new large-scale datasets in Section~\ref{sec:res}. 

\item \textbf{\uline{D2/W1}: In addition to the model performance, the model complexity, training time, and memory costs are also important to be evaluated.}

In our design space, the training time and memory costs depend highly on the sampling scope, batch size, and dataset characteristics, making it demanding to conduct a thorough empirical analysis of module-level costs. Previous work ~\cite{chen2022bottleneck} has provided a detailed analysis of the module-level training time and memory costs for some models (TGN~\cite{tgn}, TGAT~\cite{tgat}, etc.). This can be considered an analysis of several single points in our design space. We also added the following noteworthy points to Section ~\ref{sec:res} from the cost-effectiveness perspective: For neighbor sampling, the overhead is almost negligible($1\%-2\%$ of training time) with our parallel GPU sampler. For node memory, the memory costs depend on the number of nodes in the dataset and the dimension of the hidden embeddings. This cost is usually limited because of the comparatively small number of nodes on temporal graphs. We have further compared models that use node memory with models that sample large neighborhoods instead of using node memory in Figure ~\ref{fig:mem_time}. For the node aggregator modules, we have added the analysis of the theoretical complexity as well as a comparison of training time and memory costs in Section ~\ref{subsubsec:aggr}.  

\item \textbf{\uline{D3/W3}: There are recent works that train TGN models on large-scale graphs, as described in the related work section. It is important to include them as compared models or at least discuss whether the works have introduced optimized modules (which may enlarge the design space). In the second case, some empirical analysis is needed to evaluate the optimization effects.}

We have summarized recent works that train TGN models on large-scale graphs in several aspects and then discussed how their optimized models are related to our framework.
\begin{enumerate}
    \item Some works use adaptive sampling to capture information with fewer neighbors~\cite{astgn, taser}, which can be included as extra methods in our evaluation of node sampling. However, as these works bring significant communication and computation overhead and a much larger design space, we did not include them in our framework. We have added a discussion about these works in Section~\ref{subsec:modular}.
    \item Some works introduce parallel techniques and distributed frameworks for training~\cite{disttgl, gnnflow}. These works are orthogonal to our work, as the distributed techniques may be applied after the TGNN model is constructed under our framework. Some acceleration techniques are specific to certain types of GNNs ((TGL~\cite{tgl} for memory-based TGNNs, and TGOpt~\cite{tgopt} for accelerating TGAT~\cite{tgat})). It is difficult to include these works as comparison as they are beyond our modular TGNN framework and highly specific. We have added further clarification about this in Section ~\ref{sec:related}. Nonetheless, for future efforts to evaluate the optimizations, we provided guidelines in Section ~\ref{subsec:hs} for multi-GPU configurations to support future integration and evaluation of distributed optimizations.
\end{enumerate}


\item \textbf{\uline{D4}: In the related work section, citations should not be used as a subject of a sentence.}

We thank the reviewer for his careful review and have made the changes to the citation formats accordingly.

\item \shepherding{ \textbf{ \uline{AD1}: Additional Comments:
While the revision paper has included two large graphs in the datasets, i.e., GDELT and SuperUser. Most of the experimental results are obtained on a subset of small graph datasets.
When checking the figures in the experiments, it seems that different figures use a subset of the listed datasets without discussion about the choice of the subset. The two largest datasets are only used in the results of Figure 5 and 6. Please discuss the choice of datasets for different experiments, and present whether the conclusions hold on all the 9 datasets. }}


\shepherding{We used different subsets of datasets in the discussion mainly for clarity and conciseness, but we ran all experiments on all datasets and confirmed that the conclusions hold on all datasets. We showed results from all datasets where there is little for visualization (Figure ~\ref{fig:mem}). In other figures, the number and combination of datasets we chose are based on several principals: For universal results that one module outperforms another, we selected commonly used datasets with which readers may be more familiar; for results that require a discussion about the module-dataset interplay, we selected a diverse combination of datasets to cover the module performance under different dataset patterns; for analysis about scalability, we select datasets of all scales. We acknowledge that this may cause some confusion and question on the universality of the results, and we have made efforts to account for the selection of datasets in Section ~\ref{sec:res}}.    

\item \shepherding{ \textbf{ \uline{AD2}: Additional Comments:
Figure 4 shows the results on UCI, Wiki, Reddit, and Flights, while the caption mentions LastFM. Please proofread the experiments to ensure the correctness of all the results.}}


\shepherding{We thank the reviewer for the attention. We have corrected the mistake in the caption and aligned the caption and the figure.}   
    
\end{enumerate}

\subsection{Response to Reviewer \#3}
\begin{enumerate}[label=\arabic*:, leftmargin=0.44cm]

\item \textbf{\uline{D1/W1}: Most of the used datasets are bipartite graphs in social networks. It would be more convincing if more temporal graphs in diverse domains, such as transportation road networks, are used for comparison.}

Due to limitations in dataset collection, transportation networks are usually pre-processed to discrete-time dynamic graphs (DTDGs) without rich node or edge features, which are not in the scope of this work. Despite the limitations in transportation networks, our experimental settings include one transportation network \textit{Flights}~\cite{edgebank}.

Besides social networks, we also have datasets from other domains, including user action dataset (\textit{MOOC}~\cite{jodie}), transportation network(\textit{Flights}~\cite{edgebank}), and non-bipartite social networks on various topics(\textit{UCI}~\cite{opsahl2009clustering}, \textit{CollegeMsg}~\cite{panzarasa2009patterns}, and \textit{LASTFM}~\cite{jodie}).

To make our experiments more convincing, we have further added two large-scale graph datasets in different domains: GDELT as a global events network~\cite{tgl} and SuperUser as a user temporal network~\cite{orca}.

\item \textbf{\uline{D2/W3}: Only one uniform sampling approach is used, and more other approaches for performance evaluation are fair.}

In our evaluation of sampling methods, we cover uniform and most recent sampling (\textbf{uni} and \textbf{MR}), which are the two mainstream sampling strategies on dynamic graphs. Previous work also evaluated inverse-time sampling, but it performs worse than uniform sampling~\cite{tgat}. We have added additional notes on this in Section ~\ref{subsec:modular}.

On top of \textbf{uni}/\textbf{MR} sampling, recent works~\cite{taser, astgn} have proposed some adaptive neighbor sampling techniques. However, these methods introduce tremendous computation and communication overheads. We have added discussions on this in Section ~\ref{subsec:modular}. We leave the work to compare \textbf{uni}, \textbf{MR}, \textbf{uni}+adaptive, and \textbf{MR}+adaptive to future works.

\textbf{\uline{W2}: Some details, such as TGNN pipeline and model implementation are needed.}

We have detailed the TGNN pipeline and implementations according to the comments. Specifically, we have added one paragraph about the complete TGNN pipeline at the start of Section ~\ref{subsec:imple}, explaining how modules are employed to construct the training framework. We have also added details to clarify the module implementation in later parts of Section ~\ref{subsec:imple}.

\item \textbf{\uline{D3}: The three questions seem to be also applicable to general GNN models, not unique to TGNN. Not sure these questions are the most important and it will be meaningful to give some discussion to demonstrate the importance of such questions.}

While the three research questions presented in Section ~\ref{sec:intro} are important to both TGNNs and GNNs, the emphasis differs between static and temporal graphs due to their distinct characteristics, tasks, and models. For instance, the node memory module is unique to the TGNN domain. We believe that discussions within the TGNN domain yield some domain-specific knowledge. 
As our comparison work focuses on achieving optimality where high predictive accuracy and resource efficiency are balanced (as stated in Section ~\ref{sec:intro}), most important questions are the cost-effectiveness and universality of the TGNN modules, as explored by our research questions in Section ~\ref{sec:intro}.

\end{enumerate}
